Task-Specific Preconditioner for Cross-Domain Few-Shot Learning

Cross-Domain Few-Shot Learning~(CDFSL) methods typically parameterize models with task-agnostic and task-specific parameters. To adapt task-specific parameters, recent approaches have utilized fixed optimization strategies, despite their potential sub-optimality across varying domains or target tasks. To address this issue, we propose a novel adaptation mechanism called Task-Specific Preconditioned gradient descent~(TSP). Our method first meta-learns Domain-Specific Preconditioners~(DSPs) that capture the characteristics of each meta-training domain, which are then linearly combined using task-coefficients to form the Task-Specific Preconditioner. The preconditioner is applied to gradient descent, making the optimization adaptive to the target task. We constrain our preconditioners to be positive definite, guiding the preconditioned gradient toward the direction of steepest descent. Empirical evaluations on the Meta-Dataset show that TSP achieves state-of-the-art performance across diverse experimental scenarios.

==> Latex_files/99_checklist.tex <==
\clearpage
\onecolumn
\begin{center}
    \textbf{\Large Check list}
\end{center}
This paper:
Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes)\\
Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes)\\
Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes)\\

Does this paper make theoretical contributions? (yes)\\
If yes, please complete the list below.
All assumptions and restrictions are stated clearly and formally. (yes)\\
All novel claims are stated formally (e.g., in theorem statements). (yes)\\
Proofs of all novel claims are included. (yes)\\
Proof sketches or intuitions are given for complex and/or novel results. (no)\\
Appropriate citations to theoretical tools used are given. (no)\\
All theoretical claims are demonstrated empirically to hold. (no)\\
All experimental code used to eliminate or disprove claims is included. (no)\\

Does this paper rely on one or more datasets? (yes)\\
If yes, please complete the list below.\\
A motivation is given for why the experiments are conducted on the selected datasets (yes)\\
All novel datasets introduced in this paper are included in a data appendix. (NA)\\
All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (NA)\\
All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes)\\
All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes)\\
All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (NA)\\

Does this paper include computational experiments? (yes)\\
If yes, please complete the list below.\\
Any code required for pre-processing data is included in the appendix. (yes)\\
All source code required for conducting and analyzing the experiments is included in a code appendix. (yes)\\
All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes)\\
All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes)\\
If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes)\\
This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes)\\
This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes)\\
This paper states the number of algorithm runs used to compute each reported result. (yes)\\
Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes)\\
The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes)\\
This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes)\\
This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes)
